ADATIME: A Benchmarking Suite for Domain Adaptation on Time Series Data

Unsupervised domain adaptation methods aim to generalize well on unlabeled test data that may have a different (shifted) distribution from the training data. Such methods are typically developed on image data, and their application to time series data is less explored. Existing works on time series domain adaptation suffer from inconsistencies in evaluation schemes, datasets, and backbone neural network architectures. Moreover, labeled target data are often used for model selection, which violates the fundamental assumption of unsupervised domain adaptation. To address these issues, we develop a benchmarking evaluation suite (AdaTime) to systematically and fairly evaluate different domain adaptation methods on time series data. Specifically, we standardize the backbone neural network architectures and benchmarking datasets, while also exploring more realistic model selection approaches that can work with no labeled data or just a few labeled samples. Our evaluation includes adapting state-of-the-art visual domain adaptation methods to time series data as well as the recent methods specifically developed for time series data. We conduct extensive experiments to evaluate 11 state-of-the-art methods on five representative datasets spanning 50 cross-domain scenarios. Our results suggest that with careful selection of hyper-parameters, visual domain adaptation methods are competitive with methods proposed for time series domain adaptation. In addition, we find that hyper-parameters could be selected based on realistic model selection approaches. Our work unveils practical insights for applying domain adaptation methods on time series data and builds a solid foundation for future works in the field. The code is available at \href{https://github.com/emadeldeen24/AdaTime}{github.com/emadeldeen24/AdaTime}.

==> Tables/URL_table.tex <==
\begin{table}[h]
\caption{The URLs for the codes we implemented in our AdaTime framework}
\centering
\begin{NiceTabular}{@{}l|cl@{}}
\toprule
Method & Code Available & Code link \\ \midrule
DDC & \checkmark & https://github.com/syorami/DDC-transfer-learning \\
Deep Coral & \checkmark & https://github.com/SSARCandy/DeepCORAL \\
HoMM & \checkmark & https://github.com/chenchao666/HoMM-Master \\
MMDA & \xmark & our implementation \\
DSAN & \checkmark & https://github.com/easezyc/deep-transfer-learning/ \\
DANN & \checkmark & https://github.com/fungtion/DANN \\
CDAN & \checkmark & https://github.com/thuml/CDAN \\
DIRT-T & \checkmark & https://github.com/RuiShu/dirt-t \\
CoDATS & \checkmark & https://github.com/floft/codats \\
AdvSKM & \checkmark & https://github.com/jarheadjoe/Adv-spec-ker-matching \\
SASA & \checkmark & https://github.com/DMIRLAB-Group/SASA \\
\bottomrule
\end{NiceTabular}
\label{tbl:urls}
\end{table}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
